Stability Analysis and Performance Evaluation of Mixed-Precision Runge-Kutta Methods

Additive Runge-Kutta methods designed for preserving highly accurate solutions in mixed-precision computation were proposed and analyzed in 4. These specially designed methods use reduced precision for the implicit computations and full precision for the explicit computations. In this work we analyze the stability properties of these methods and their sensitivity to the low precision rounding errors, and demonstrate their performance in terms of accuracy and efficiency. We develop codes in FORTRAN and Julia to solve nonlinear systems of ODEs and PDEs using the mixed precision additive Runge-Kutta (MP-ARK) methods. The convergence, accuracy, runtime, and energy consumption of these methods is explored. We show that for a given level of accuracy, suitably chosen MP-ARK methods may provide significant reductions in runtime.

==> tables.tex <==
\begin{tabular}{ |c|c|c|c|c|c|  }
 \hline
 \multicolumn{6}{|c|}{IM-1p Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.000711 & 0.000127 & 0.000068& 0.000114& 0.000066& 0.000066\\
 0.005860 & 0.000494 & 0.000268& 0.000438& 0.000180& 0.000173\\
 0.029061 & 0.003237 & 0.001754& 0.002614& 0.000938& 0.000974\\
 0.200017 & 0.018010 & 0.010076& 0.012969& 0.004921& 0.004857\\
 \hline
 \multicolumn{6}{|c|}{SDIRK-3p Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.001312 & 0.000154 & 0.000106 & 0.000104 & 0.000061 & 0.000062\\
 0.005928 & 0.000849 & 0.000656 & 0.000445 & 0.000224 & 0.000246\\
 0.031965 & 0.005722 & 0.004847 & 0.003261 & 0.002162 & 0.002074\\
 0.253049 & 0.045016 & 0.031873 & 0.018709 & 0.009515 & 0.009710\\
 \hline
 \multicolumn{6}{|c|}{Novel Method 4s3pA Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.001543 & 0.000273 & 0.000194& 0.000199& 0.000134& 0.000136\\
 0.011115 & 0.001399 & 0.000811& 0.000915& 0.000340& 0.000378\\
 0.062933 & 0.007696 & 0.005559& 0.004917& 0.002095& 0.002157\\
 0.430059 & 0.052646 & 0.035969& 0.026183& 0.009849& 0.009585\\
 \hline
\end{tabular}

\begin{tabular}{ |c|c|c|c|c|c|  }
 \hline
 \multicolumn{6}{|c|}{IM-1p Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.049744 & 0.036462 & 0.044959 & 0.050281 & 0.036926 & 0.032813\\
 0.159118 & 0.050097 & 0.049841 & 0.045911 & 0.035938 & 0.036951\\
 0.910398 & 0.094299 & 0.070422 & 0.078406 & 0.057129 & 0.053747\\
 6.473018 & 0.577672 & 0.310851 & 0.427819 & 0.153808 & 0.148559\\
 \hline
 \multicolumn{6}{|c|}{SDIRK-3p Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.071838 & 0.046496 & 0.039599 & 0.047351 & 0.034021 & 0.038892\\
 0.165441 & 0.051184 & 0.051196 & 0.041333 & 0.054175 & 0.051135\\
 1.022189 & 0.162341 & 0.136706 & 0.091602 & 0.083764 & 0.075671\\
 8.298050 & 1.292672 & 1.028257 & 0.608995 & 0.282971 & 0.297912\\
 \hline
 \multicolumn{6}{|c|}{Novel Method 4s3pA Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.064453 & 0.042297 & 0.047803 & 0.038269 & 0.048828 & 0.039978\\
 0.327233 & 0.070776 & 0.057043 & 0.066992 & 0.042712 & 0.043274\\
 2.083210 & 0.217529 & 0.153747 & 0.131237 & 0.072473 & 0.074780\\
 14.091297 & 1.713252 & 1.131870 & 0.859373 & 0.297594 & 0.285473\\
 \hline
\end{tabular}

%\begin{tabular}{ |c|c|c|c|c|c|  }
% \hline
%\multicolumn{6}{|c|}{IM-1p Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000160 & 0.000123 & 0.000067& 0.000123& 0.000069& 0.000068\\
% 0.001475 & 0.000521 & 0.000214& 0.000509& 0.000206& 0.000211\\
% 0.010053 & 0.003126 & 0.001250& 0.003063& 0.001201& 0.001211\\
% 0.073585 & 0.022139 & 0.007639& 0.021594& 0.007134& 0.007334\\
% \hline
% \multicolumn{6}{|c|}{SDIRK-3p Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000289 & 0.000118 & 0.000068& 0.000128& 0.000061& 0.000060\\
% 0.001474 & 0.000617 & 0.000333& 0.000589& 0.000308& 0.000308\\
% 0.010242 & 0.004347 & 0.002977& 0.004053& 0.002709& 0.002718\\
% 0.092578 & 0.034395 & 0.019270& 0.031540& 0.016639& 0.017124\\
% \hline
% \multicolumn{6}{|c|}{Novel Method 4s3pA Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000321 & 0.000291 & 0.000163& 0.000248& 0.000161& 0.000163\\
% 0.003142 & 0.001245 & 0.000482& 0.001132& 0.000475& 0.000479\\
% 0.020565 & 0.006853 & 0.002965& 0.007067& 0.002869& 0.002930\\
% 0.140042 & 0.049135 & 0.018296& 0.047340& 0.017068& 0.017110\\
% \hline
%\end{tabular}
